It's All In the Teacher: Zero-Shot Quantization Brought Closer to the Teacher

Model quantization is considered as a promising method to greatly reduce the resource requirements of deep neural networks. To deal with the performance drop induced by quantization errors, a popular method is to use training data to fine-tune quantized networks. In real-world environments, however, such a method is frequently infeasible because training data is unavailable due to security, privacy, or confidentiality concerns. Zero-shot quantization addresses such problems, usually by taking information from the weights of a full-precision teacher network to compensate the performance drop of the quantized networks. In this paper, we first analyze the loss surface of state-of-the-art zero-shot quantization techniques and provide several findings. In contrast to usual knowledge distillation problems, zero-shot quantization often suffers from 1) the difficulty of optimizing multiple loss terms together, and 2) the poor generalization capability due to the use of synthetic samples. Furthermore, we observe that many weights fail to cross the rounding threshold during training the quantized networks even when it is necessary to do so for better performance. Based on the observations, we propose AIT, a simple yet powerful technique for zero-shot quantization, which addresses the aforementioned two problems in the following way: AIT i) uses a KL distance loss only without a cross-entropy loss, and ii) manipulates gradients to guarantee that a certain portion of weights are properly updated after crossing the rounding thresholds. Experiments show that AIT outperforms the performance of many existing methods by a great margin, taking over the overall state-of-the-art position in the field.

==> figs/hessian/hessianGDFQ.tex <==
\begin{tikzpicture}

			
\pgfplotscreateplotcyclelist{custom}{%https://tex.stackexchange.com/questions/134346/different-marker-shape-for-pgf-tikz
solid, thick, mark size=2pt, every mark/.append style={solid, thick, fill=color1}, mark=*\\%
solid, thick, mark size=2pt, every mark/.append style={solid, thick, fill=color1}, mark=square*\\%
solid, thick, mark size=2pt, every mark/.append style={solid, thick, fill=color1}, mark=diamond*\\%
solid, thick, mark size=2pt, every mark/.append style={solid, thick, fill=color2}, mark=*\\%
solid, thick, mark size=2pt, every mark/.append style={solid, thick, fill=color2}, mark=square*\\%
solid, thick, mark size=2pt, every mark/.append style={solid, thick, fill=color2}, mark=diamond*\\%
%loosely dotted, thick, mark size=3pt, every mark/.append style={solid, fill=gray}, mark=triangle*\\%
solid, thick, mark size=3pt, every mark/.append style={solid, thick, fill=color2}, mark=square*\\%
solid, thick, mark size=3pt, every mark/.append style={solid, thick, fill=color1}, mark=*\\%
dotted, thick, mark size=3pt, every mark/.append style={solid, thick, fill=color1}, mark=otimes*\\%
densely dotted, thick, mark size=3pt, every mark/.append style={solid, fill=color1}, mark=diamond*\\%
loosely dotted, thick, mark size=3pt, every mark/.append style={solid, fill=color1}, mark=triangle*\\%
solid, thick, mark size=3pt, every mark/.append style={solid, thick, fill=color2}, mark=*\\%
dotted, thick, mark size=3pt, every mark/.append style={solid, thick, fill=color2}, mark=otimes*\\%
densely dotted, thick, mark size=3pt, every mark/.append style={solid, fill=color2}, mark=diamond*\\%
loosely dotted, thick, mark size=3pt, every mark/.append style={solid, fill=color2}, mark=triangle*\\%
dotted, thick, mark size=3pt, every mark/.append style={solid, thick, fill=gray}, mark=otimes*\\%
densely dotted, thick, mark size=3pt, every mark/.append style={solid, fill=gray}, mark=diamond*\\%
loosely dotted, thick, mark size=3pt, every mark/.append style={solid, fill=gray}, mark=triangle*\\%
solid, thick, mark size=3pt, every mark/.append style={solid, thick, fill=gray}, mark=*\\%
dashed, thick, every mark/.append style={solid, fill=color5},mark=otimes*\\%
loosely dashed, thick, every mark/.append style={solid, fill=gray},mark=*\\%
densely dashed, thick, every mark/.append style={solid, fill=gray},mark=square*\\%
dashdotted, thick, every mark/.append style={solid, fill=gray},mark=otimes*\\%
dashdotdotted, thick, every mark/.append style={solid},mark=star\\%
densely dashdotted,thick, every mark/.append style={solid, fill=gray},mark=diamond*\\%
}

\centering
\begin{axis}[
%font=\footnotesize\rmfamily,
%title style={yshift=-1.5mm},
%axis, % dual axis plot
width=\textwidth, 
height=3cm,
xmajorticks=true,
ymajorgrids,
%ymax=8,
ymin = 0,
%ytick={1,3,5,7},
%xtick={0,1,2,3,4},
%xticklabels={2,4,8,16,32},
xlabel = {Epoch},
xlabel shift=-.3em,
xlabel near ticks,
ylabel near ticks,
xlabel style={at={(ticklabel cs:0.9)},font =\rmfamily\scriptsize},
x tick label style = {font =\scriptsize, text width = 1.4cm, align = center, anchor = north},
ylabel={Log(Tr(H))},
ylabel style = {font=\scriptsize, yshift=0cm},
y tick label style = {font =\scriptsize, anchor = east, 
 /pgf/number format/fixed, %, xshift=.6cm
},
legend cell align={left},
legend style={draw=none, fill=none, at={(0.54,1.0), font=\scriptsize},
anchor=south,legend columns=3,
/tikz/every even column/.append style={column sep=0.5cm}},
% legend image code/.code={%
%   \draw[#1] (0cm,-0.1cm) rectangle (0.2cm,0.1cm);
% }
]  

\addplot[mark=none,thick,color=olivegreen] table [x=epoch, y=CEGDFQ] {figs/hessian/hessiandata.txt};\addlegendentry{CE}
\addplot[mark=none,thick,color=blue] table [x=epoch, y=KLGDFQ] {figs/hessian/hessiandata.txt};\addlegendentry{KL}




\end{axis}
\end{tikzpicture}  

==> tables/perf0.tex <==
\begin{table*}[]
    \centering
    \footnotesize
    

    
    % \def\arraystretch{0.9}% 
    %\begin{tabular}{c|p{6mm}|p{6mm}|p{6mm}|l|c|c|c|c}
    \resizebox{\textwidth}{!}
    {
    \begin{tabular}{x{1.5cm}|c|c|c|cc|cc|cc}
    \toprule
    Dataset & \makecell{Model\\(FP32 Acc.)} & Bits & ZeroQ & 
    GDFQ & \makecell{GDFQ\\{\footnotesize+\aname}}  &
    
    Qimera & \makecell{Qimera\\{\footnotesize+\aname}}  
    \\
      \midrule
      \multirow{2}{*}{Cifar-10} &  ResNet-20 & 3w3a  &  79.30 & 92.13 & 90.25 (+3.00) & 89.58 & 88.69 (-3.44)  & 00.0 & 91.26 (-0.87) \\
                                & (93.89)    & 4w4a  & 91.3   & 93.36 & 93.38 (+3.00) & 92.75 & 92.79 (-0.59) & 00.0 & \textbf{93.46  (+0.08)} \\
      \midrule
      \multirow{2}{*}{Cifar-100} & ResNet-20  & 3w3a & 47.45 & 60.42 &  63.39 (+3.00) & 62.74 & 62.99 (-0.40) & 00.0 & \textbf{65.10 (+1.71)} \\
                                 &(70.33) & 4w4a & 65.61 & 68.70$^*$ & 66.12 (+3.00)  & 67.51 & 67.78 (-0.92)  & 00.0 & \textbf{69.02 (+0.32)} \\
      

      \midrule
       \multirow{6}{*}{ImageNet} &  ResNet-18   & 3w3a  &  22.58 & 52.64 &60.60 (+3.00) & 58.90 & 61.72 (+1.12) & 00.0 & \textbf{63.84 (+3.24)} \\
                             &  (71.47) & 4w4a & 59.26 & 64.54 & 68.40 (+3.00) & 68.05 & 68.67 (+0.27) &  00.0 & \textbf{69.29 (+0.89)} \\
                                 & ResNet-50 & 3w3a & {\color{white}0}8.38 & 53.02$^*$ & 52.12 (+3.00) & 51.80 & 59.25 (+6.24) &  00.0 & \textbf{66.25 (+3.23)} \\
                                  &  (77.73) & 4w4a & 48.12 & 73.38$^*$ & 71.89 (+3.00) & 70.99 & 71.57 (-1.81) & 00.0 & \textbf{75.32 (+1.94)} \\
    
                            & MobileNetV2 &  3w3a & 10.96 & {\color{white}0}0.10$^{\dagger}$ &59.43 (+3.00) & 57.23 & 59.99 (+0.56)&  00.0 & \textbf{61.62 (+2.19)} \\
                                  & (73.03)  & 4w4a & 59.88 & 62.35 & 68.11 (+3.00) & 67.61 & 68.83 (+0.72) & 00.0 & \textbf{70.45 (+2.34)} \\

               \bottomrule
          \multicolumn{10}{r}{\small$^*$ Highest among the baselines\ \  $^\dagger$Did not converge} \\
    \end{tabular}}
        \caption{Comparison on \aname with data-free quantization schemes.\JL{all numbers are placeholders. expecting about 4-5\% improvement overall.}}
    \label{tab:exp}
\end{table*}

==> tables/sense.tex <==
\begin{table}[]
\renewcommand{\arraystretch}{0.8}
    \centering
    %\footnotesize
    
    
    % \def\arraystretch{0.9}% 
    %\begin{tabular}{c|p{6mm}|p{6mm}|p{6mm}|l|c|c|c|c}
    %\resizebox{\textwidth}{!}
    
    \begin{tabular}{ccccc}
    \toprule
    \multirow{2}{*}{$\rho$} & \multicolumn{1}{c}{Cifar-100} & \multicolumn{1}{c}{ImageNet} \\
    \cmidrule(lr){3-3}\cmidrule(lr){2-2}
     & ResNet-20 & ResNet-18  \\
    \midrule



0.005	&	63.01	&	57.95	\\
					
0.001	&	65.80	&	60.11	\\
					
0.0005	&	65.41	&	64.48	\\
					
0.0001	&	65.04	&	65.51	\\
					
0.00005	&	65.30	&	65.92	\\

      \bottomrule
    \end{tabular} 
    \vspace{-2mm}
    \caption{Sensitivity Analysis.}
    \vspace{-4mm}
    \label{tab:sense}
\end{table}

==> tables/sensemore.tex <==
\begin{table}[]

    \centering
    %\footnotesize
    
    
    % \def\arraystretch{0.9}% 
    %\begin{tabular}{c|p{6mm}|p{6mm}|p{6mm}|l|c|c|c|c}
    %\resizebox{\textwidth}{!}
    
    \begin{tabular}{cccccc}
    \toprule
    \multicolumn{2}{c}{Param.}&\multicolumn{1}{c}{Cifar-100} & \multicolumn{1}{c}{ImageNet} \\
    \cmidrule(lr){3-3}\cmidrule(lr){4-4}
    $\rho$&decay & ResNet-20 & ResNet-18  \\
    \midrule


%\multirow{2}{*}{0.05}	&	\ding{52} 	&	59.16	&	59.49	\\
%	&	\ding{56} 	&	58.61	&	57.12	\\
%\multirow{2}{*}{0.01}	&	\ding{52} 	&	59.08	&	58.94	\\
%	&	\ding{56} 	&	58.89	&	57.00	\\
\multirow{2}{*}{0.005}	&	\ding{52} 	&	63.01	&	57.95	\\
	&	\ding{56} 	&	63.56	&	58.95	\\
\multirow{2}{*}{0.001}	&	\ding{52} 	&	65.80	&	60.11	\\
	&	\ding{56} 	&	65.43	&	60.63	\\
\multirow{2}{*}{0.0005}	&	\ding{52} 	&	65.41	&	64.48	\\
	&	\ding{56} 	&	65.50	&	63.83	\\
\multirow{2}{*}{0.0001}	&	\ding{52} 	&	65.04	&	65.51	\\
	&	\ding{56} 	&	65.12	&	65.60	\\
\multirow{2}{*}{0.00005}	&	\ding{52} 	&	65.30	&	65.92	\\
	&	\ding{56} 	&	65.19	&	65.76	\\

      \bottomrule
    \end{tabular} 
    
    \caption{Sensitivity Analysis.}
    \label{tab:sense}
\end{table}
